Towards More Human-like AI Communication: A Review of Emergent Communication Research

In the recent shift towards human-centric AI, the need for machines to accurately use natural language has become increasingly important. While a common approach to achieve this is to train large language models, this method presents a form of learning misalignment where the model may not capture the underlying structure and reasoning humans employ in using natural language, potentially leading to unexpected or unreliable behavior. Emergent communication (Emecom) is a field of research that has seen a growing number of publications in recent years, aiming to develop artificial agents capable of using natural language in a way that goes beyond simple discriminative tasks and can effectively communicate and learn new concepts. In this review, we present Emecom under two aspects. Firstly, we delineate all the common proprieties we find across the literature and how they relate to human interactions. Secondly, we identify two subcategories and highlight their characteristics and open challenges. We encourage researchers to work together by demonstrating that different methods can be viewed as diverse solutions to a common problem and emphasize the importance of including diverse perspectives and expertise in the field. We believe a deeper understanding of human communication is crucial to developing machines that can accurately use natural language in human-machine interactions.

==> tables/new_bib_list.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{lscape}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{landscape}
\tiny  % Switch from 12pt to 11pt; otherwise, table won't fit

\setlength\tabcolsep{1.5pt} % default value: 6pt
\begin{longtable}{|c|cc|ccccc|cc|cccc|cc|}

\label{tab:list}\\
\hline
Citation & \multicolumn{2}{c|}{Theory of mind} & \multicolumn{5}{c|}{Interaction Type} & \multicolumn{2}{c|}{Game Environment} & \multicolumn{4}{c|}{Update Algorithm} & \multicolumn{2}{c|}{Methodology} \\ \hline
\endfirsthead
%
\multicolumn{16}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\hline
Citation & Modeling & Influencing & In. Coop & Out. Coop & Comp & Pop. & Iter. & Com-goal & Com-aid & Reinforce & Gumble & Supervised & other & Symbolic & Natural\\ \hline
\endhead
%
 & Modeling & Influencing & In. Coop & Out. Coop & Comp & Pop. & Iter. & Com-goal & Com-aid & Reinforce & Gumble & Supervised & other & Symbolic & Natural \\ \hline
\cite{Kirby2014} &  &  & x &  &  &  & x & x &  &  &  &  &  &  & x \\ \hline
\cite{Andreas2016} & x & x & x &  &  &  &  &  &  &  &  & x &  &  & x \\ \hline
\cite{Foerster2016} &  &  & x &  &  &  &  & x &  & x &  &  &  & x &  \\ \hline
\cite{Lazaridou2016} &  &  & x &  &  &  &  & Ref &  &  &  & IML &  & x & x \\ \hline
\cite{Nakamura2016} & x &  & x & x & x &  &  &  & SG &  &  &  &  & x &  \\ \hline
\cite{Sukhbaatar2016} &  &  & x & x & x &  &  &  & x & x &  & x &  & x &  \\ \hline
\cite{Das2017} &  &  & x &  &  &  &  & VQA &  & x &  & DG &  &  & x \\ \hline
\cite{Evtimova2017} & x &  & x &  &  &  &  & Ref &  & x &  &  &  & x &  \\ \hline
\cite{Foerster2017} & x & x &  &  &  &  &  &  &  & x &  &  &  &  &  \\ \hline
\cite{Havrylov2017} &  &  &  &  &  &  &  & Ref &  & x & x &  &  & x & x \\ \hline
\cite{Kong2017} &  &  & x &  &  &  &  &  & x & x &  &  &  & x &  \\ \hline
\cite{Kottur2017} &  &  & x &  &  &  &  & TnT &  & x &  &  &  & x &  \\ \hline
\cite{Lee2017} &  &  & x &  &  &  &  & Ref &  & x &  & x &  &  & x \\ \hline
\cite{Lowe2017} & x &  & x & x & x &  &  & x & nav & x & x &  &  & x &  \\ \hline
\cite{abs-1804-02341} & x &  & x &  &  &  &  & Ref &  & x &  & ToM &  & x &  \\ \hline
\cite{abs-1810-08647} & x & x & x &  &  &  &  &  & SG & x &  & ToM &  & x &  \\ \hline
\cite{Bouchacourt2018} &  &  & x &  &  &  &  & Ref &  & x &  &  &  & x &  \\ \hline
\cite{Cao2018} & x &  & x & x &  & x &  &  & neg & x &  &  &  & x &  \\ \hline
\cite{Grover2018} & x &  & x & x &  &  &  &  & nav & x &  &  & UnS & x &  \\ \hline
\cite{Lazaridou2018} &  &  & x &  &  &  &  & Red &  & x &  &  &  & x &  \\ \hline
\cite{Mordatch2018} &  &  & x &  &  &  &  &  & nav & x &  &  &  & x &  \\ \hline
\cite{Raileanu2018} & x &  & x &  &  &  &  &  &  & x &  & ToM &  &  &  \\ \hline
\cite{abs-1809-00549} & x &  & x &  &  &  &  & x & x & x &  & ToM &  & x &  \\ \hline
\cite{abs-1910-05291} &  &  & x & x &  & x & x &  & x & x & x &  &  & x &  \\ \hline
\cite{abs-1910-06079} &  &  & x &  &  &  &  & x &  & x & x &  &  & x &  \\ \hline
\cite{abs-1912-05676} &  &  &  &  &  &  &  & x & nav & x &  &  &  & x &  \\ \hline
\cite{abs-1912-06208} &  &  & x & x &  & x & x & x &  &  &  & x &  & x &  \\ \hline
\cite{Bouchacourt2019} &  &  &  &  &  &  &  &  &  & x &  &  &  & x &  \\ \hline
\cite{Chaabouni2019} &  &  & x &  &  &  & x &  & nav &  &  & x &  & x &  \\ \hline
\cite{Das2019} & x & x & x & x & x &  &  &  & nav & x &  & x &  & x &  \\ \hline
\cite{Fitzgerald2019} &  &  & x &  &  & x &  & Ref &  & x &  &  &  & x &  \\ \hline
\cite{Graesser2019} &  &  & x &  &  & x & x & Ref &  & x &  & x &  & x &  \\ \hline
\cite{JaquesLHGOSLF19} & x & x & x & x & x &  &  &  & x & x &  & ToM &  &  &  \\ \hline
\cite{Lee2019} &  &  & x &  &  &  &  & MT &  & x &  & DG &  &  & x \\ \hline
\cite{Li2019} &  &  & x &  &  & x & x & Ref &  & x &  &  &  & x &  \\ \hline
\cite{Lowe2019a} &  &  & x &  &  & x & x & TnT &  & x &  &  &  & x &  \\ \hline
\cite{Omidshafiei2019} &  &  & x & x &  &  &  &  & x & x & x &  &  & x &  \\ \hline
\cite{Resnick2019} &  &  &  &  &  &  &  &  &  &  & x &  &  &  &  \\ \hline
\cite{Rodriguez2019} & x &  & x & x &  & x &  & Ref &  & x &  & ToM &  & x &  \\ \hline
\cite{abs-2001-07752} & x &  & x &  &  &  &  & Ref &  & x &  &  &  & x &  \\ \hline
\cite{abs-2002-01365} &  &  & x &  &  &  & x & Ref &  & x &  & x &  & x &  \\ \hline
\cite{abs-2003-12694} &  &  & x &  &  &  & x & Ref &  & x & x & x &  &  & x \\ \hline
\cite{abs-2010-02975} &  &  & x & x &  &  & x & x &  & x & x & x &  &  & x \\ \hline
\cite{Bachrach2020} &  &  & x & x &  &  &  &  &  & x &  & x &  &  &  \\ \hline
\cite{Chaabouni2020} &  &  & x &  &  &  &  & Ref &  & x & x &  &  & x &  \\ \hline
\cite{Cogswell2020} &  &  &  &  &  &  &  & VQA &  & x & x & x &  &  & x \\ \hline
\cite{HawkinsKSG20} & x & x & x &  &  &  &  & Ref &  &  &  & x &  &  & x \\ \hline
\cite{Lazaridou2020} &  &  & x &  &  &  &  & Ref &  & x &  & x &  &  & x \\ \hline
\cite{Li2020} &  &  & x &  &  &  &  & Ref &  &  & x & x &  &  & x \\ \hline
\cite{Liang2020} &  &  & x &  & x &  &  & TnT &  & x &  &  &  & x &  \\ \hline
\cite{Lowe2020} &  &  & x &  &  & x & x & Ref &  &  & x & x &  &  & x \\ \hline
\cite{Xie2020} & x & x &  &  &  &  &  &  &  & x &  & x &  &  &  \\ \hline
\cite{abs-2001-03361} &  &  & x & x &  & x & x & Ref &  &  & x & x & EvL & x &  \\ \hline
\cite{abs-2107-05697} & x & x & x &  &  & x &  & Ref & nav & x & x & x &  &  & x \\ \hline
\cite{abs-2110-05422} &  &  & x &  &  & x &  & Ref &  &  & x & x &  &  & x \\ \hline
\cite{Brandizzi2021} & x &  & x & x & x &  &  &  & SG & x &  &  &  & x &  \\ \hline
\cite{abs-2204-12982} &  &  & x & x &  & x &  & Ref &  & x & x &  &  & x &  \\ \hline
\cite{ChaabouniSATTDM22} &  &  & x & x &  & x &  & x &  & x &  & ToM &  & x &  \\ \hline
\cite{abs-2106-04258} &  &  & x &  &  &  &  & Ref &  &  & x & x &  & x &  \\ \hline
\cite{abs-2004-03420} &  &  & x &  &  &  &  & Ref &  &  &  & x &  & x &  \\ \hline
\cite{GuptaLFKP19} &  &  & x &  &  & x & x & Ref &  & x & x & x &  & x & x \\ \hline
\cite{abs-1905-12561} &  &  & x &  &  &  &  & Ref &  & x & x &  &  & x & x \\ \hline
\cite{abs-2012-10776} &  &  & x &  &  &  &  & Ref &  & x & x &  &  & x &  \\ \hline
\cite{abs-1912-05304} &  &  & x &  &  &  &  &  & x & x &  &  & UnS & x &  \\ \hline
\cite{abs-2005-05441} &  &  & x & x & x &  &  &  & x & x & x &  &  & x &  \\ \hline
\cite{abs-1911-06992} &  &  & x & x & x &  &  &  & x & x &  &  &  & x &  \\ \hline
\cite{KharitonovCBB20} &  &  & x &  &  &  &  &  & x & x & x &  & SCG & x &  \\ \hline
\end{longtable}
\end{landscape}

